What Do You Get When You Cross Beam Search with Nucleus Sampling?

We combine beam search with the probabilistic pruning technique of nucleus sampling to create two deterministic nucleus search algorithms for natural language generation. The first algorithm, p-exact search, locally prunes the next-token distribution and performs an exact search over the remaining space. The second algorithm, dynamic beam search, shrinks and expands the beam size according to the entropy of the candidate's probability distribution. Despite the probabilistic intuition behind nucleus search, experiments on machine translation and summarization benchmarks show that both algorithms reach the same performance levels as standard beam search.

==> TAB2_norm.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Peam  max rank} & &  \textbf{>= 5} & \textbf{< 5}  \\
\midrule
\textbf{Dynamic-Beam} & 0.6  &  42.4 & 33.0 \\ 
\textbf{Beam} & 5  &  42.3 & 33.7\\ 
\midrule
\#examples &   &  2680 & 323 \\ 
\bottomrule
\end{tabular}
\caption{Length normalized generations scores of subword level WMT14 EN-FR. \uri{Needed? if so fix formatting of course and more importantly this is length normalized - so make sure its the same as the main table} \omer{Let's get the unnormalized numbers.} \omer{caption}}
\label{tab:norm_maxrank}
\end{table}



==> TAB_5_norm.tex <==
\begin{table*}[]
\small
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Search}} & \multirow{2}{*}{\textbf{Hyperparameter}} &  \textbf{WMT'14} & \textbf{IWSLT'14} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{XSUM}}} \\
\multirow{2}{*}{\textbf{Algorithm}} & \multirow{2}{*}{\textbf{(}$k$ \textbf{or} $p$\textbf{)}} & \textbf{EN-FR} & \textbf{DE-EN (Char)} & & & \\
 & & \textbf{BLEU} & \textbf{BLEU} & \textbf{ROUGE1} & \textbf{ROUGE2} & \textbf{ROUGE-L} \\
\midrule
Beam & 5  &  41.0 & \textbf{34.1} & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 

     \midrule
     \multirow{9}{*}{$P$-Exact - max(k)=5} & 0.1  &  40.3 & 33.3 & 42.6 & 20.4 & 35.5 \\ 
& 0.2  &  40.3 & 33.3 & 42.8 & 20.5 & 35.6 \\ 
& 0.3  &  40.5 & 33.4 & 43.2 & 21.0 & 36.0 \\ 
& 0.4  &  40.7 & 33.4 & 43.4 & 21.4 & 36.3 \\ 
& 0.5  &  40.9 & 33.6 & 43.5 & 21.6 & 36.5 \\ 
& 0.6  &  \textbf{41.2} & 33.7 & 43.6 & 21.7 & 36.5 \\ 
& 0.7  &  41.1 & 33.9 & \textbf{43.7} & 21.8 & \textbf{36.6} \\ 
& 0.8  &  \textbf{41.2} & 34.0 & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 
& 0.9  &  41.0 & \textbf{34.1} & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 

     \midrule
     \multirow{9}{*}{Dynamic-Beam - max(k)=5} & 0.1  &  40.2 & 33.3 & 42.6 & 20.4 & 35.5 \\ 
& 0.2  &  40.3 & 33.3 & 42.7 & 20.5 & 35.6 \\ 
& 0.3  &  40.5 & 33.4 & 43.1 & 20.9 & 36.0 \\ 
& 0.4  &  40.6 & 33.4 & 43.2 & 21.3 & 36.2 \\ 
& 0.5  &  40.8 & 33.4 & 43.4 & 21.6 & 36.4 \\ 
& 0.6  &  41.0 & 33.8 & 43.6 & 21.8 & 36.5 \\ 
& 0.7  &  41.1 & 34.0 & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 
& 0.8  &  41.0 & 34.0 & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 
& 0.9  &  41.0 & \textbf{34.1} & \textbf{43.7} & \textbf{21.9} & \textbf{36.6} \\ 

    \bottomrule
\end{tabular}
\caption{Fixed beam size of 5: Length normalized generations scores of subword level WMT14 EN-FR, character level IWSLT14 DE-EN, and XSUM using different search algorithms.  \omer{caption} \uri{add 2,3,4 and underlines}}
\label{tab:norm_5}
\end{table*}
